Continuous-Time Flows for Efficient Inference and Density Estimation

Two fundamental problems in unsupervised learning are efficient inference for latent-variable models and robust density estimation based on large amounts of unlabeled data. Algorithms for the two tasks, such as normalizing flows and generative adversarial networks (GANs), are often developed independently. In this paper, we propose the concept of {\em continuous-time flows} (CTFs), a family of diffusion-based methods that are able to asymptotically approach a target distribution. Distinct from normalizing flows and GANs, CTFs can be adopted to achieve the above two goals in one framework, with theoretical guarantees. Our framework includes distilling knowledge from a CTF for efficient inference, and learning an explicit energy-based distribution with CTFs for density estimation. Both tasks rely on a new technique for distribution matching within amortized learning. Experiments on various tasks demonstrate promising performance of the proposed CTF framework, compared to related techniques.

==> Definitions.tex <==
\newcommand{\eat}[1]{}

\def\KL{\textsf{KL}}

\newcommand{\Cy}{\Ccal_y}
\renewcommand{\l}{\boldsymbol{\ell}}
\renewcommand{\S}
{\!\!\,\includegraphics[height=1em]{figs/arcsinh}\!\!}
\def\Gt{\widetilde{G}}
\def\ah{\widehat{a}}
\def\ahb{\mathbf{\ah}}
\def\at{\widetilde{a}}
\def\atb{\mathbf{\at}}
\def\yh{\widehat{y}}
\def\yt{\widetilde{y}}
\def\ytb{\mathbf{\yt}}
\def\yhb{\mathbf{\yh}}
\def\zh{\widehat{z}}
\def\zt{\widetilde{z}}
\def\ztb{\mathbf{\zt}}
\def\zhb{\mathbf{\zh}}
\def\g{\mathbf{g}}
\def\bah{\mathbf{\widehat{a}}}
\RequirePackage{latexsym}
\RequirePackage{amsmath}
%\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}

\definecolor{magenta}{cmyk}{0,1,0,0}
\definecolor{mygreen}{rgb}{.1,1,.1}
\newcommand{\Magenta}[1]{\color{magenta}{#1}\color{black}}
\newcommand{\Blue}[1]{\textcolor{blue}{#1}}
%\newcommand{\Green}[1]{\color{OliveGreen}{#1}}
\newcommand{\Green}[1]{\textcolor{mygreen}{#1}}
\newcommand{\Red}[1]{\textcolor{red}{#1}}
\newcommand{\Cyan}[1]{\textcolor{cyan}{#1}}
\newcommand{\Orange}[1]{\textcolor{orange}{#1}}
\newcommand{\Brown}[1]{\textcolor{brown}{#1}}
\newcommand{\Ref}[1]{\hfill\Green{[#1]}}
\DeclareMathOperator{\arginf}{arg\,inf}
%\newcommand{\alert}[1]{\Red{\bf {#1}}}

\newcommand{\rmd}{\mathrm{d}} % use italics only for variable

\newcommand{\Tr}{^\mathsf{T}} % sf looks nicer than rm


%%% MW %%%%

\newcommand{\mnote}[1]{{\bf\large *}\marginpar{\Magenta{#1}}}
\newcommand{\dnote}[1]{{\bf\large +}\marginpar{\tiny#1}}
\ifx\note\undefined
\newcommand{\note}[1]{{\bf \Magenta{#1}}}
\else
\renewcommand{\note}[1]{{\bf \Magenta{#1}}}
\fi

\def\x{\mathbf{x}}
\def\a{\mathbf{a}}
\def\y{\mathbf{y}}
\def\z{\mathbf{z}}
\def\w{\mathbf{w}}
\def\t{\boldsymbol{\theta}}
\def\R{\mathbb{R}}

%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\DeclareMathOperator{\ab}{\mathbf{a}}
\DeclareMathOperator{\bb}{\mathbf{b}}
\DeclareMathOperator{\cbb}{\mathbf{c}}
\DeclareMathOperator{\db}{\mathbf{d}}
\DeclareMathOperator{\eb}{\mathbf{e}}
\DeclareMathOperator{\fb}{\mathbf{f}}
\DeclareMathOperator{\gb}{\mathbf{g}}
\DeclareMathOperator{\hb}{\mathbf{h}}
\DeclareMathOperator{\ib}{\mathbf{i}}
\DeclareMathOperator{\jb}{\mathbf{j}}
\DeclareMathOperator{\kb}{\mathbf{k}}
\DeclareMathOperator{\lb}{\mathbf{l}}
\DeclareMathOperator{\mb}{\mathbf{m}}
\DeclareMathOperator{\nbb}{\mathbf{n}}
\DeclareMathOperator{\ob}{\mathbf{o}}
\DeclareMathOperator{\pb}{\mathbf{p}}
\DeclareMathOperator{\qb}{\mathbf{q}}
\DeclareMathOperator{\rb}{\mathbf{r}}
\DeclareMathOperator{\sbb}{\mathbf{s}}
\DeclareMathOperator{\tb}{\mathbf{t}}
\DeclareMathOperator{\ub}{\mathbf{u}}
\DeclareMathOperator{\vb}{\mathbf{v}}
\DeclareMathOperator{\wb}{\mathbf{w}}
\DeclareMathOperator{\xb}{\mathbf{x}}
 \DeclareMathOperator{\yb}{\mathbf{y}}
\DeclareMathOperator{\zb}{\mathbf{z}}

\DeclareMathOperator{\pr}{\mathrm{p}}

\DeclareMathOperator{\deltab}{\boldsymbol{\delta}}

\DeclareMathOperator{\atilde}{\tilde{\ab}}
\DeclareMathOperator{\btilde}{\tilde{\bb}}
\DeclareMathOperator{\ctilde}{\tilde{\cb}}
\DeclareMathOperator{\dtilde}{\tilde{\db}}
\DeclareMathOperator{\etilde}{\tilde{\eb}}
\DeclareMathOperator{\ftilde}{\tilde{\fb}}
\DeclareMathOperator{\gtilde}{\tilde{\gb}}
\DeclareMathOperator{\htilde}{\tilde{\hb}}
\DeclareMathOperator{\itilde}{\tilde{\ib}}
\DeclareMathOperator{\jtilde}{\tilde{\jb}}
\DeclareMathOperator{\ktilde}{\tilde{\kb}}
\DeclareMathOperator{\ltilde}{\tilde{\lb}}
\DeclareMathOperator{\mtilde}{\tilde{\mb}}
\DeclareMathOperator{\ntilde}{\tilde{\nbb}}
\DeclareMathOperator{\otilde}{\tilde{\ob}}
%
\DeclareMathOperator{\qtilde}{\tilde{\qb}}
\DeclareMathOperator{\rtilde}{\tilde{\rb}}
\DeclareMathOperator{\stilde}{\tilde{\sbb}}
\DeclareMathOperator{\ttilde}{\tilde{\tb}}
\DeclareMathOperator{\utilde}{\tilde{\ub}}
\DeclareMathOperator{\vtilde}{\tilde{\vb}}
\DeclareMathOperator{\wtilde}{\tilde{\wb}}
\DeclareMathOperator{\xtilde}{\tilde{\xb}}
\DeclareMathOperator{\ytilde}{\tilde{\yb}}
\DeclareMathOperator{\ztilde}{\tilde{\zb}}

\DeclareMathOperator{\abar}{\bar{\ab}}
\DeclareMathOperator{\bbar}{\bar{\bb}}
\DeclareMathOperator{\cbar}{\bar{\cb}}
\DeclareMathOperator{\dbar}{\bar{\db}}
\DeclareMathOperator{\ebar}{\bar{\eb}}
\DeclareMathOperator{\fbar}{\bar{\fb}}
\DeclareMathOperator{\gbar}{\bar{\gb}}
\DeclareMathOperator{\hbbar}{\bar{\hb}}
\DeclareMathOperator{\ibar}{\bar{\ib}}
\DeclareMathOperator{\jbar}{\bar{\jb}}
\DeclareMathOperator{\kbar}{\bar{\kb}}
\DeclareMathOperator{\lbar}{\bar{\lb}}
\DeclareMathOperator{\mbar}{\bar{\mb}}
\DeclareMathOperator{\nbar}{\bar{\nbb}}
\DeclareMathOperator{\obar}{\bar{\ob}}
\DeclareMathOperator{\pbar}{\bar{\pb}}
\DeclareMathOperator{\qbar}{\bar{\qb}}
\DeclareMathOperator{\rbar}{\bar{\rb}}
\DeclareMathOperator{\sbar}{\bar{\sbb}}
\DeclareMathOperator{\tbar}{\bar{\tb}}
\DeclareMathOperator{\ubar}{\bar{\ub}}
\DeclareMathOperator{\vbar}{\bar{\vb}}
\DeclareMathOperator{\wbar}{\bar{\wb}}
\DeclareMathOperator{\xbar}{\bar{\xb}}
\DeclareMathOperator{\ybar}{\bar{\yb}}
\DeclareMathOperator{\zbar}{\bar{\zb}}

\DeclareMathOperator{\Ab}{\mathbf{A}}
\DeclareMathOperator{\Bb}{\mathbf{B}}
\DeclareMathOperator{\Cb}{\mathbf{C}}
\DeclareMathOperator{\Db}{\mathbf{D}}
\DeclareMathOperator{\Eb}{\mathbf{E}}
\DeclareMathOperator{\Fb}{\mathbf{F}}
\DeclareMathOperator{\Gb}{\mathbf{G}}
\DeclareMathOperator{\Hb}{\mathbf{H}}
\DeclareMathOperator{\Ib}{\mathbf{I}}
\DeclareMathOperator{\Jb}{\mathbf{J}}
\DeclareMathOperator{\Kb}{\mathbf{K}}
\DeclareMathOperator{\Lb}{\mathbf{L}}
\DeclareMathOperator{\Mb}{\mathbf{M}}
\DeclareMathOperator{\Nb}{\mathbf{N}}
\DeclareMathOperator{\Ob}{\mathbf{O}}
\DeclareMathOperator{\Pb}{\mathbf{P}}
\DeclareMathOperator{\Qb}{\mathbf{Q}}
\DeclareMathOperator{\Rb}{\mathbf{R}}
\DeclareMathOperator{\Sbb}{\mathbf{S}}
\DeclareMathOperator{\Tb}{\mathbf{T}}
\DeclareMathOperator{\Ub}{\mathbf{U}}
\DeclareMathOperator{\Vb}{\mathbf{V}}
\DeclareMathOperator{\Wb}{\mathbf{W}}
\DeclareMathOperator{\Xb}{\mathbf{X}}
\DeclareMathOperator{\Yb}{\mathbf{Y}}
\DeclareMathOperator{\Zb}{\mathbf{Z}}

\DeclareMathOperator{\Abar}{\bar{A}}
\DeclareMathOperator{\Bbar}{\bar{B}}
\DeclareMathOperator{\Cbar}{\bar{C}}
\DeclareMathOperator{\Dbar}{\bar{D}}
\DeclareMathOperator{\Ebar}{\bar{E}}
\DeclareMathOperator{\Fbar}{\bar{F}}
\DeclareMathOperator{\Gbar}{\bar{G}}
\DeclareMathOperator{\Hbar}{\bar{H}}
\DeclareMathOperator{\Ibar}{\bar{I}}
\DeclareMathOperator{\Jbar}{\bar{J}}
\DeclareMathOperator{\Kbar}{\bar{K}}
\DeclareMathOperator{\Lbar}{\bar{L}}
\DeclareMathOperator{\Mbar}{\bar{M}}
\DeclareMathOperator{\Nbar}{\bar{N}}
\DeclareMathOperator{\Obar}{\bar{O}}
\DeclareMathOperator{\Pbar}{\bar{P}}
\DeclareMathOperator{\Qbar}{\bar{Q}}
\DeclareMathOperator{\Rbar}{\bar{R}}
\DeclareMathOperator{\Sbar}{\bar{S}}
\DeclareMathOperator{\Tbar}{\bar{T}}
\DeclareMathOperator{\Ubar}{\bar{U}}
\DeclareMathOperator{\Vbar}{\bar{V}}
\DeclareMathOperator{\Wbar}{\bar{W}}
\DeclareMathOperator{\Xbar}{\bar{X}}
\DeclareMathOperator{\Ybar}{\bar{Y}}
\DeclareMathOperator{\Zbar}{\bar{Z}}

\DeclareMathOperator{\Abbar}{\bar{\Ab}}
\DeclareMathOperator{\Bbbar}{\bar{\Bb}}
\DeclareMathOperator{\Cbbar}{\bar{\Cb}}
\DeclareMathOperator{\Dbbar}{\bar{\Db}}
\DeclareMathOperator{\Ebbar}{\bar{\Eb}}
\DeclareMathOperator{\Fbbar}{\bar{\Fb}}
\DeclareMathOperator{\Gbbar}{\bar{\Gb}}
\DeclareMathOperator{\Hbbar}{\bar{\Hb}}
\DeclareMathOperator{\Ibbar}{\bar{\Ib}}
\DeclareMathOperator{\Jbbar}{\bar{\Jb}}
\DeclareMathOperator{\Kbbar}{\bar{\Kb}}
\DeclareMathOperator{\Lbbar}{\bar{\Lb}}
\DeclareMathOperator{\Mbbar}{\bar{\Mb}}
\DeclareMathOperator{\Nbbar}{\bar{\Nb}}
\DeclareMathOperator{\Obbar}{\bar{\Ob}}
\DeclareMathOperator{\Pbbar}{\bar{\Pb}}
\DeclareMathOperator{\Qbbar}{\bar{\Qb}}
\DeclareMathOperator{\Rbbar}{\bar{\Rb}}
\DeclareMathOperator{\Sbbar}{\bar{\Sb}}
\DeclareMathOperator{\Tbbar}{\bar{\Tb}}
\DeclareMathOperator{\Ubbar}{\bar{\Ub}}
\DeclareMathOperator{\Vbbar}{\bar{\Vb}}
\DeclareMathOperator{\Wbbar}{\bar{\Wb}}
\DeclareMathOperator{\Xbbar}{\bar{\Xb}}
\DeclareMathOperator{\Ybbar}{\bar{\Yb}}
\DeclareMathOperator{\Zbbar}{\bar{\Zb}}

\DeclareMathOperator{\Ahat}{\widehat{A}}
\DeclareMathOperator{\Bhat}{\widehat{B}}
\DeclareMathOperator{\Chat}{\widehat{C}}
\DeclareMathOperator{\Dhat}{\widehat{D}}
\DeclareMathOperator{\Ehat}{\widehat{E}}
\DeclareMathOperator{\Fhat}{\widehat{F}}
\DeclareMathOperator{\Ghat}{\widehat{G}}
\DeclareMathOperator{\Hhat}{\widehat{H}}
\DeclareMathOperator{\Ihat}{\widehat{I}}
\DeclareMathOperator{\Jhat}{\widehat{J}}
\DeclareMathOperator{\Khat}{\widehat{K}}
\DeclareMathOperator{\Lhat}{\widehat{L}}
\DeclareMathOperator{\Mhat}{\widehat{M}}
\DeclareMathOperator{\Nhat}{\widehat{N}}
\DeclareMathOperator{\Ohat}{\widehat{O}}
\DeclareMathOperator{\Phat}{\widehat{P}}
\DeclareMathOperator{\Qhat}{\widehat{Q}}
\DeclareMathOperator{\Rhat}{\widehat{R}}
\DeclareMathOperator{\Shat}{\widehat{S}}
\DeclareMathOperator{\That}{\widehat{T}}
\DeclareMathOperator{\Uhat}{\widehat{U}}
\DeclareMathOperator{\Vhat}{\widehat{V}}
\DeclareMathOperator{\What}{\widehat{W}}
\DeclareMathOperator{\Xhat}{\widehat{X}}
\DeclareMathOperator{\Yhat}{\widehat{Y}}
\DeclareMathOperator{\Zhat}{\widehat{Z}}

\DeclareMathOperator{\Abhat}{\widehat{\Ab}}
\DeclareMathOperator{\Bbhat}{\widehat{\Bb}}
\DeclareMathOperator{\Cbhat}{\widehat{\Cb}}
\DeclareMathOperator{\Dbhat}{\widehat{\Db}}
\DeclareMathOperator{\Ebhat}{\widehat{\Eb}}
\DeclareMathOperator{\Fbhat}{\widehat{\Fb}}
\DeclareMathOperator{\Gbhat}{\widehat{\Gb}}
\DeclareMathOperator{\Hbhat}{\widehat{\Hb}}
\DeclareMathOperator{\Ibhat}{\widehat{\Ib}}
\DeclareMathOperator{\Jbhat}{\widehat{\Jb}}
\DeclareMathOperator{\Kbhat}{\widehat{\Kb}}
\DeclareMathOperator{\Lbhat}{\widehat{\Lb}}
\DeclareMathOperator{\Mbhat}{\widehat{\Mb}}
\DeclareMathOperator{\Nbhat}{\widehat{\Nb}}
\DeclareMathOperator{\Obhat}{\widehat{\Ob}}
\DeclareMathOperator{\Pbhat}{\widehat{\Pb}}
\DeclareMathOperator{\Qbhat}{\widehat{\Qb}}
\DeclareMathOperator{\Rbhat}{\widehat{\Rb}}
\DeclareMathOperator{\Sbhat}{\widehat{\Sb}}
\DeclareMathOperator{\Tbhat}{\widehat{\Tb}}
\DeclareMathOperator{\Ubhat}{\widehat{\Ub}}
\DeclareMathOperator{\Vbhat}{\widehat{\Vb}}
\DeclareMathOperator{\Wbhat}{\widehat{\Wb}}
\DeclareMathOperator{\Xbhat}{\widehat{\Xb}}
\DeclareMathOperator{\Ybhat}{\widehat{\Yb}}
\DeclareMathOperator{\Zbhat}{\widehat{\Zb}}

\DeclareMathOperator{\Acal}{\mathcal{A}}
\DeclareMathOperator{\Bcal}{\mathcal{B}}
\DeclareMathOperator{\Ccal}{\mathcal{C}}
\DeclareMathOperator{\Dcal}{\mathcal{D}}
\DeclareMathOperator{\Ecal}{\mathcal{E}}
\DeclareMathOperator{\Fcal}{\mathcal{F}}
\DeclareMathOperator{\Gcal}{\mathcal{G}}
\DeclareMathOperator{\Hcal}{\mathcal{H}}
\DeclareMathOperator{\Ical}{\mathcal{I}}
\DeclareMathOperator{\Jcal}{\mathcal{J}}
\DeclareMathOperator{\Kcal}{\mathcal{K}}
\DeclareMathOperator{\Lcal}{\mathcal{L}}
\DeclareMathOperator{\Mcal}{\mathcal{M}}
\DeclareMathOperator{\Ncal}{\mathcal{N}}
\DeclareMathOperator{\Ocal}{\mathcal{O}}
\DeclareMathOperator{\Pcal}{\mathcal{P}}
\DeclareMathOperator{\Qcal}{\mathcal{Q}}
\DeclareMathOperator{\Rcal}{\mathcal{R}}
\DeclareMathOperator{\Scal}{\mathcal{S}}
\DeclareMathOperator{\Tcal}{\mathcal{T}}
\DeclareMathOperator{\Ucal}{\mathcal{U}}
\DeclareMathOperator{\Vcal}{\mathcal{V}}
\DeclareMathOperator{\Wcal}{\mathcal{W}}
\DeclareMathOperator{\Xcal}{\mathcal{X}}
\DeclareMathOperator{\Ycal}{\mathcal{Y}}
\DeclareMathOperator{\Zcal}{\mathcal{Z}}

\DeclareMathOperator{\Atilde}{\widetilde{A}}
\DeclareMathOperator{\Btilde}{\widetilde{B}}
\DeclareMathOperator{\Ctilde}{\widetilde{C}}
\DeclareMathOperator{\Dtilde}{\widetilde{D}}
\DeclareMathOperator{\Etilde}{\widetilde{E}}
\DeclareMathOperator{\Ftilde}{\widetilde{F}}
\DeclareMathOperator{\Gtilde}{\widetilde{G}}
\DeclareMathOperator{\Htilde}{\widetilde{H}}
\DeclareMathOperator{\Itilde}{\widetilde{I}}
\DeclareMathOperator{\Jtilde}{\widetilde{J}}
\DeclareMathOperator{\Ktilde}{\widetilde{K}}
\DeclareMathOperator{\Ltilde}{\widetilde{L}}
\DeclareMathOperator{\Mtilde}{\widetilde{M}}
\DeclareMathOperator{\Ntilde}{\widetilde{N}}
\DeclareMathOperator{\Otilde}{\widetilde{O}}
\DeclareMathOperator{\Ptilde}{\widetilde{P}}
\DeclareMathOperator{\Qtilde}{\widetilde{Q}}
\DeclareMathOperator{\Rtilde}{\widetilde{R}}
\DeclareMathOperator{\Stilde}{\widetilde{S}}
\DeclareMathOperator{\Ttilde}{\widetilde{T}}
\DeclareMathOperator{\Utilde}{\widetilde{U}}
\DeclareMathOperator{\Vtilde}{\widetilde{V}}
\DeclareMathOperator{\Wtilde}{\widetilde{W}}
\DeclareMathOperator{\Xtilde}{\widetilde{X}}
\DeclareMathOperator{\Ytilde}{\widetilde{Y}}
\DeclareMathOperator{\Ztilde}{\widetilde{Z}}


%%%%%%%% Widely accepted definitions %%%%%%%%%%%%%%%

\DeclareMathOperator{\CC}{\mathbb{C}} % Complex numbers
\DeclareMathOperator{\EE}{\mathbb{E}} % Expectation
\DeclareMathOperator{\KK}{\mathbb{K}} % Arbitrary field
\DeclareMathOperator{\MM}{\mathbb{M}} % Median
\DeclareMathOperator{\NN}{\mathbb{N}} % Natural numbers
\DeclareMathOperator{\PP}{\mathbb{P}} % Probability
\DeclareMathOperator{\QQ}{\mathbb{Q}} % Rationals
\DeclareMathOperator{\RR}{\mathbb{R}} % Real numbers
\DeclareMathOperator{\ZZ}{\mathbb{Z}} % Integers

\DeclareMathOperator{\one}{\mathbf{1}}  % Identity
\DeclareMathOperator{\zero}{\mathbf{0}} % Zero

\DeclareMathOperator*{\mini}{\mathop{\mathrm{minimize}}}
\DeclareMathOperator*{\maxi}{\mathop{\mathrm{maximize}}}
\DeclareMathOperator*{\argmin}{\mathop{\mathrm{argmin}}}
\DeclareMathOperator*{\argsup}{\mathop{\mathrm{argsup}}}
\DeclareMathOperator*{\arcsinh}{\mathop{\mathrm{arcsinh}}}
\DeclareMathOperator*{\limit}{\mathop{\mathrm{limit}}}
\DeclareMathOperator*{\argmax}{\mathop{\mathrm{argmax}}}
\DeclareMathOperator{\sgn}{\mathop{\mathrm{sign}}}
\DeclareMathOperator{\tr}{\mathop{\mathrm{tr}}}
\DeclareMathOperator{\rank}{\mathop{\mathrm{rank}}}
\DeclareMathOperator{\traj}{\mathop{\mathrm{Traj}}}
\DeclareMathOperator{\diag}{diag}

%%%%%%%% Bold Greek Letters %%%%%%%%%%%%%%%
\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}
\newcommand{\Thetab}{{\bm{\Theta}}}
\newcommand{\thetab}{{\bm{\theta}}}
\newcommand{\xib}{{\bm{\xi}}}
\newcommand{\Xib}{{\bm{\Xi}}}
\newcommand{\zetab}{{\bm{\zeta}}}
\newcommand{\alphab}{{\bm{\alpha}}}
\newcommand{\taub}{{\bm{\tau}}}
\newcommand{\etab}{{\bm{\eta}}}


\DeclareMathOperator{\alphahat}{\widehat{\alpha}}
%%%%%%%% Mess around with LaTeX %%%%%%%%%%%%%%%

%% Some style files might actually define these variables.
%% So don't mess with them if they are already defined

\ifx\BlackBox\undefined
\newcommand{\BlackBox}{\rule{1.5ex}{1.5ex}}  % end of proof
\fi

\ifx\proof\undefined
\newenvironment{proof}{\par\noindent{\bf Proof\ }}{\hfill\BlackBox\\[2mm]}
\fi

\ifx\theorem\undefined
\newtheorem{theorem}{Theorem}
\fi
\ifx\example\undefined
\newtheorem{example}{Example}
\fi
\ifx\lemma\undefined
\newtheorem{lemma}[theorem]{Lemma}
\fi

\ifx\corollary\undefined
\newtheorem{corollary}[theorem]{Corollary}
\fi

\ifx\definition\undefined
\newtheorem{definition}[theorem]{Definition}
\fi

\ifx\proposition\undefined
\newtheorem{proposition}[theorem]{Proposition}
\fi

\ifx\remark\undefined
\newtheorem{remark}[theorem]{Remark}
\fi

\ifx\conjecture\undefined
\newtheorem{conjecture}[theorem]{Conjecture}
\fi

\ifx\factoid\undefined
\newtheorem{factoid}[theorem]{Fact}
\fi

\ifx\axiom\undefined
\newtheorem{axiom}[theorem]{Axiom}
\fi

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%brackets
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}

\newcommand{\ea}{\emph{et al. }}
\newcommand{\eg}{\emph{e.g. }}
\newcommand{\ie}{\emph{i.e., }}

\newcommand{\vishy}[1]{{\bf[#1--VISHY]}}
\newcommand{\tim}[1]{{\bf[#1 --TIM]}}

%Logic
%\newcommand{\implies}{\Rightarrow}
%\newcommand{\iff}{\Leftrightarrow}
\newcommand{\goesto}{\rightarrow}
\newcommand{\suchthat}{\ensuremathmode{\text{ such that }}}
\newcommand{\st}{\suchthat}

%%%%%%%% Specific symbols for this project %%%%%%%%%%%%%%%

% upright names for matrices --don't use for single-letter function names!
\newcommand{\A}{\mathbf{A}}
\newcommand{\As}{\mathbf{A}^{\!\!*}}
\newcommand{\B}{\mathbf{B}}
\newcommand{\Bs}{\mathbf{B}^{*}}

% p and variants
\newcommand{\p}{\mathbf{p}}
\newcommand{\pp}{\p^{\prime}}
\newcommand{\ps}{\p^*}
\newcommand{\po}{\p_0}
\newcommand{\pos}{\p_{0}^{*}}
\newcommand{\poi}{[\p_{0}]_i}
\newcommand{\pii}{\p_{i}}
\newcommand{\pip}{\p_{i}^{\prime}}
\newcommand{\pis}{\p_{i}^{*}}
\newcommand{\pBar}{\bar{\p}}
\newcommand{\pohat}{\widehat{\p}_0}
\newcommand{\phat}{\widehat{\p}}
\newcommand{\psBar}{\bar{\p}^{*}}
\newcommand{\pbb}{\p_{\bb}}

% mu and variants
\newcommand{\mub}{{\bm{\mu}}}
\newcommand{\ms}{\m^{*}}
\newcommand{\mo}{\m_0}
\newcommand{\mh}{\widehat{\m}}
\newcommand{\mBar}{\bar{\m}}
\newcommand{\msBar}{\bar{\m}^{*}}

% Bold mu_B
\newcommand{\mB}{\m_{\B}}
\newcommand{\mBBar}{\bar{\m}_{\B}}
% mu_1
\newcommand{\mone}{\mu_{\mathbf{1}}}
\newcommand{\mones}{\mu_{\mathbf{1}}^{*}}
\newcommand{\monesBar}{\bar{\mu}^{*}_\mathbf{1}}

% q and variants
\newcommand{\q}{\mathbf{q}}
\newcommand{\qs}{\q^{*}}
\newcommand{\qii}{\q_{i}}

% b and variants
\newcommand{\bone}{\mathbf{b_1}}
%\newcommand{\bone}{\ones}

% c and variants
\newcommand{\cs}{\cbb^{*}}

% Functions
\newcommand{\Fs}{F^{*}}
\newcommand{\Gs}{G^{*}}
\newcommand{\Hs}{H^{*}}
\newcommand{\fsi}{f_{i}^{*}}

% Dual Spaces
\DeclareMathOperator{\Xcals}{\Xcal^{*}}
\DeclareMathOperator{\Mcals}{\Mcal^{*}}

% set and domain concepts
\DeclareMathOperator{\ri}{\mathrm{ri}}      % Relative interior
\DeclareMathOperator{\intr}{\mathrm{int}}   % Interior
\DeclareMathOperator{\bd}{\mathrm{bdry}}      % Boundary (see RocWet98)
\DeclareMathOperator{\dom}{\mathrm{dom}}    % Effective Domain
\DeclareMathOperator{\epi}{\mathrm{epi}}    % Epigraph
\DeclareMathOperator{\ran}{\mathrm{range}}  % Range of an operator

\newcommand{\by}{\times}

% gradient: \grad{F}{\m}
\newcommand{\grad}[2]{\nabla #1 \left( #2 \right) }
\newcommand{\hess}[2]{\nabla^2 #1 \left( #2 \right) }
\newcommand{\grd}{\nabla} % simpler version!
\newcommand{\breg}[1]{\Delta #1} % Bregman divergence

% subgradient: \subgrad{F}{\m}
\newcommand{\subgrad}[2]{\partial #1 \left( #2 \right) }
% subdiferential
\newcommand{\subdiff}{\partial}

% Vector of all ones
\newcommand{\ones}{\eb}

% Sum from i equal 1 to n
\newcommand{\sumin}{\sum_{i=1}^{n}}

% Deformed logarithm wrt \phi
\newcommand{\lphi}{\log_{\phi}}

% function k_{\phi}
\newcommand{\kphi}{k_{\phi}}

% reparam for dual log
%\newcommand{\phib}{\phi^{\bullet}}
\newcommand{\phib}{\pmb{\phi}}
%\newcommand{\psib}{\psi^{\bullet}}
\newcommand{\psib}{\pmb{\psi}}

% Deformed exponential wrt \phi
\newcommand{\ephi}{\exp_{\phi}}

% One over deformed exponential wrt \phi
\newcommand{\ephib}{\exp^{\bullet}_{\phi}}

% Gradient of deformed exponential wrt \phi
\newcommand{\ephip}{\nabla_{x} \exp_{\phi}}

% Gradient of t-exponential wrt \phi
\newcommand{\ephit}{\nabla_{x} \exp_{t}}

% Deformed logarithm wrt \psi
\newcommand{\lpsi}{\log_{\psi}}

% One over deformed logarithm wrt \psi
\newcommand{\lpsib}{\log^{\bullet}_{\psi}}
\newcommand{\lphib}{\log^{\bullet}_{\phi}}

%composition needed for conjugate--formerly combo
\newcommand{\lcirce}{\lpsi \circ \ephib}

% S and related
\newcommand{\Sp}{S_{\phi}}
\newcommand{\Sps}{S^{*}_{\phi}}
\newcommand{\smp}{s_{\phi}}
\newcommand{\smpp}{s^{\prime}_{\phi}}
\newcommand{\smps}{s^{*}_{\phi}}

% T
\newcommand{\T}{T^{*}}
\DeclareMathOperator{\tp}{\tilde{p}}
\DeclareMathOperator{\tq}{\tilde{q}}
\DeclareMathOperator{\tg}{\tilde{g}}
\DeclareMathOperator{\tmu}{\tilde{\mu}}
\DeclareMathOperator{\tthe}{\tilde{\theta}}
\DeclareMathOperator{\ttheb}{{\bf \tilde{\theta}}}
\DeclareMathOperator{\tmc}{\widehat{\Mcal}}
\DeclareMathOperator{\tv}{\tilde{v}}


\DeclareMathOperator{\Remp}{R_{\text{emp}}}

\DeclareMathOperator{\tsallis}{\text{tsallis}}

%\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
%\newcommand{\rbr}[1]{\left(#1\right)}
%\newcommand{\cbr}[1]{\left\{#1\right\}}
%\newcommand{\nbr}[1]{\left\|#1\right\|}
%\newcommand{\abr}[1]{\left|#1\right|}
\def\ah{\widehat{a}}
\def\ahb{\mathbf{\ah}}
%\newcommand{\sbr}[1]{\left[#1\right]}
%\DeclareMathOperator*{\arginf}{\mathop{\mathrm{arginf}}}
\DeclareMathOperator*{\lnm}{\mathop{\mathbf{ln}}}
\mathchardef\Theta="7102 \mathchardef\theta="7112
\newcommand{\I}{{\mathcal{I}}}
\newcommand{\tops}{{\!\top\!}}
%\newcommand{\R}{\hbox{\bf R}}
%\newcommand{\z}{{\mathbf{z}}}
\newcommand{\vxi}{{\boldsymbol{\xi}}}
\newcommand{\vtheta}{{\boldsymbol{\theta}}}
\newcommand{\valpha}{{\boldsymbol{\alpha}}}
\newcommand{\m}{{\mathbf{m}}}
\newcommand{\tc}[2]{\textcolor{#1}{#2}}
\renewcommand{\k}{k}
\ifx\br\undefined
\newcommand{\br}{\color{red}}
\else
\renewcommand{\br}{\color{red}}
\fi
%\newcommand{\bb}{\color{blue}}
\newcommand{\brh}{\color{red}}
\newcommand{\bbh}{\color{blue}}
\newcommand{\N}{\hbox{\bf N}}
\newcommand{\Nl}{N}
\newcommand{\Proj}{P} 
\newcommand{\Hc}{{H}}             % base hypothesis class
\def\x{{\mathbf{x}}} 
\def\X{{\mathbf{X}}} 
\def\Xr{{\rm\sf X}} 
\newcommand{\eps}{\epsilon}
\def\y{{\mathbf{y}}} 
\def\w{{\mathbf{w}}} 
\def\W{{\mathbf{W}}} 
\def\RR{{\mathbf{R}}} 
\def\NN{{\mathbf{N}}} 
\newcommand{\M}{{\boldsymbol{\mu}}}
\newcommand{\ev}{\hbox{\bf v}}
\newcommand{\EV}{\hbox{\bf V}}
\def\H{{\cal{H}}}
\def\F{{\cal{F}}}
\def\Fc{{S}}
\def\Sample{{\Z}}
\def\vc{{d}}
\def\D{{\cal{D}}} 
\def\hatD{\hat{D}} 
\def\A{\hat{A}} 
\def\B{\hat{B}} 
\def\T{\hat{T}} 
\def\G{\mathcal{G}} 
\def\P{\hat{P}} 
\newcommand{\al}{\alpha}
%\newcommand{\Fs}{{\mathcal{F}}}   % feature space
\newcommand{\AL}{{\boldsymbol \alpha}}
\newcommand{\BE}{{\boldsymbol \beta}}
\newcommand{\XI}{{\boldsymbol \xi}}
%\newcommand{\sgn}{\mbox{sgn}}
\def\one{{\mathbf{1}}}
\def\hatf{\hat{f}}
\definecolor{lila}{rgb}{0.2,0,0.5}
\definecolor{rot}{rgb}{0.8,0,0}
\definecolor{blau}{rgb}{0,0,0.5}
\definecolor{gruen}{rgb}{0,0.5,0}
\definecolor{grau}{rgb}{0.85,0.8,0.85}
\definecolor{mygreen}{rgb}{.1,1,.1}

%\definecolor{Red}{rgb}{0.75,0,0}
%\definecolor{Blue}{rgb}{0,0,0.75}
%\definecolor{Green}{rgb}{0,0.75,0}
%\definecolor{Black}{rgb}{0,0,0}
%\definecolor{Orange}{rgb}{0.9,0.5,0}

%\newcommand{\Blue}[1]{\textcolor{blue}{#1}}
%\newcommand{\Green}[1]{\color{OliveGreen}{#1}}
%\newcommand{\Green}[1]{\textcolor{mygreen}{#1}}
%\newcommand{\Red}[1]{\textcolor{red}{#1}}
%\newcommand{\Orange}[1]{\textcolor{orange}{#1}}

\newcommand{\sign}{\mathop{\rm sign}}
%\newcommand{\argmin}{\mathop{\rm argmin}}
%\newcommand{\tr}{\mathop{\rm tr}}
%\newcommand{\argmax}{\mathop{\rm argmax}}
\newcommand{\Ind}{\mathop{\rm I}}
\renewcommand{\d}{{\bf d}}
\renewcommand{\l}{\Nl}
%\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Z}{\bf Z}

\newcommand{\mg}{{\rho}}
\newcommand{\MG}{{\varrho}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\ct}{{\tilde{c}}}

%\newtheorem{example}{Example} 
%\newtheorem{remark}[example]{Remark}
%\newtheorem{theorem}[example]{Theorem} 
%\newtheorem{lemma}[example]{Lemma} 
%\newtheorem{proposition}[example]{Proposition} 
%\newtheorem{corollary}[example]{Corollary}
%\newtheorem{definition}[example]{Definition}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "tit"
%%% End: 

\newcommand{\bigdot}[1]{\stackrel{\bullet}{#1}} 
\newcommand{\textc}{\color{hblue}}
\newcommand{\fgc}{\color{red}}
\newcommand{\othc}{\color{green}}
\newcommand{\bgc}{\color{black}}
\newcommand{\titc}{\bf\fgc}

%\renewcommand{{\tem}}{{\item[{\fgc $\bullet$}]}}
%\newcommand{\Ref}[1]{{\hfill\othc [#1]}}

\newcommand{\s}{\vspace*{2cm}}
\newcommand{\hs}{\vspace*{1cm}}
\ifx\bl\undefined
\newcommand{\bl}{\hspace*{0.8cm}}
\else
\renewcommand{\bl}{\hspace*{0.8cm}}
\fi
\renewcommand{\ss}{\vspace*{4cm}}
\newcommand{\fhs}{\\[2mm]}
\newcommand{\fs}{\\[4mm]}
\newcommand{\fss}{\\[8mm]}
\newcommand{\bra}[1]
       {\left. \begin{array}{c} \\[#1] \end{array} \right\} }

%\newcommand{\Lbf}{\LARGE\bf}
\newcommand{\lbf}{\large\bf}


%\newcommand{\grad}{\nabla}
\newcommand{\diff}{d\;}
%\newcommand{\qed}{$\;\;\;\Box$}
\newcommand{\equref}[1]{(\ref{#1})}
\newcommand{\sfrac}[2]{\mbox{$\frac{#1}{#2}$}}
%\newcommand{\half}{\sfrac{1}{2}}
%\newcommand{\R}{{\bf R}}
\newcommand{\eqdef}{\stackrel{\rm def}{=}}
%\newcommand{\argmin}{\mbox{argmin}}
%\renewcommand{\min}{\mbox{min}}
%\renewcommand{\max}{\mbox{max}}


\newcommand{\Wc}{{\mathcal{W}}}


%\newcommand{\vect}[1]{{\bf #1}}
\newcommand{\vect}[1]{{\mbox{\boldmath $#1$}}}
\newcommand{\squiggle}[1]{{\widetilde{#1}}}
%\newcommand{\bm}[1]{{\mbox{$\boldmath#1 $}}}

\newcommand{\dat}{{\cal{X}}}
\renewcommand{\d}{\Delta}

%\newcommand{\vb}{V_B}
\newcommand{\uo}{U_1}
\newcommand{\utp}{U_{t+1}}

%\newcommand{\zero}{\vect{0}}
%\renewcommand{\one}{\vect{1}}


\newcommand{\f}{\vect{f}}
\renewcommand{\x}{\vect{x}}
\renewcommand{\u}{\vect{u}}
%\newcommand{\bb}{\vect{b}}
\renewcommand{\y}{\vect{y}}
\newcommand{\xs}{\tilde{\x}}
\newcommand{\xo}{\x_1}
\newcommand{\xt}{\x_t}
\newcommand{\xq}{\x_q}
\newcommand{\xtp}{\x_{t+1}}
\newcommand{\xtm}{\x_{t-1}}

%\newcommand{\yt}{y_t}
\newcommand{\yq}{y_q}
%\newcommand{\yh}{\hat{y}}
\newcommand{\yht}{\yh_t}

\newcommand{\mus}{\squiggle{\mu}}
\renewcommand{\m}{\vect{\mu}}
%\newcommand{\mb}{\vect{\mu}_B}
\newcommand{\mt}{\m_t}
%\newcommand{\mr}{\m^*}
%\newcommand{\mo}{\m_1}
\newcommand{\mtp}{\m_{t+1}}
\newcommand{\mtm}{\m_{t-1}}
\newcommand{\mTp}{\m_{T+1}}
%\newcommand{\ms}{\squiggle{\m}}

%\renewcommand{\o}{{\omega}}
%\newcommand{\ot}{\o_t}
%\newcommand{\otp}{\o_{t+1}}
%\newcommand{\os}{\squiggle{\o}}
%\renewcommand{\O}{\bf{\Omega}}
%\renewcommand{\O}{\bf{g(\TH)}}
%\newcommand{\M}{\bf{M}}


\renewcommand{\th}{\vect{\theta}}
\newcommand{\tht}{\th_t}
\newcommand{\tho}{\th_1}
\newcommand{\thb}{\th_B}
\newcommand{\thtp}{\th_{t+1}}
\newcommand{\thTp}{\th_{T+1}}
\newcommand{\ths}{\squiggle{\th}}
\newcommand{\thetas}{\squiggle{\theta}}
\newcommand{\thr}{\th^*}

\newcommand{\ta}{\vect{\tau}}
\renewcommand{\w}{\vect{w}}
\newcommand{\uu}{\vect{u}}
\newcommand{\dv}{\vect{d}}
\newcommand{\vv}{\vect{v}}
\newcommand{\ws}{\squiggle{\w}}
\newcommand{\Ws}{\widetilde{\W}}
\newcommand{\wo}{\w_1}
\newcommand{\wt}{\w_t}
%\newcommand{\wb}{\w_B}
\newcommand{\vt}{\vv_t}
\newcommand{\wtp}{\w_{t+1}}
\newcommand{\vtp}{\vv_{t+1}}
\newcommand{\ttheta}{\mbox {{\boldmath $\theta$}}}
\newcommand{\zz}{\vect{z}}

\renewcommand{\TH}{\vect{\Theta}}

%\newcommand{\at}{{\alpha_t}}
\newcommand{\At}{\vect{\alpha}_t}
\newcommand{\aq}{\alpha_q}
\newcommand{\atq}{\at^q}
\newcommand{\atmq}{\a_{t-1}^q}
\newcommand{\btq}{\beta_t^q}

\newcommand{\e}{\eta}
%\newcommand{\eb}{\eta_B}
\newcommand{\ebi}{\e_B^{-1}}
\newcommand{\et}{\e_t}
\newcommand{\eT}{\e_T}
\newcommand{\eo}{\e_1}
\newcommand{\eoo}{\e_2}
\newcommand{\etp}{\e_{t+1}}
\newcommand{\eTp}{\e_{T+1}}
\newcommand{\etpp}{\e_{t+2}}
\newcommand{\eTpp}{\e_{T+2}}
\newcommand{\etm}{\e_{t-1}}
\newcommand{\eti}{\et^{-1}}
\newcommand{\eoi}{\eo^{-1}}
\newcommand{\eooi}{\eoo^{-1}}
\newcommand{\etpi}{\etp^{-1}}
\newcommand{\eTpi}{\eTp^{-1}}
\newcommand{\etppi}{\etpp^{-1}}
\newcommand{\eTppi}{\eTpp^{-1}}
\newcommand{\etmi}{\etm^{-1}}
\newcommand{\es}{\squiggle{\e}}

\renewcommand{\I}{\vect{I}}

\newcommand{\E}{\vect{\e}}
\newcommand{\Ei}{\E^{-1}}
%\newcommand{\Eb}{\E_B}
\newcommand{\Et}{\E_t}
\newcommand{\ET}{\E_T}
\newcommand{\Eo}{\E_1}
\newcommand{\Etp}{\E_{t+1}}
\newcommand{\Eti}{\Et^{-1}}
\newcommand{\Eoi}{\Eo^{-1}}
\newcommand{\Etpi}{\Etp^{-1}}
\newcommand{\Ebi}{\E_B^{-1}}
\newcommand{\Es}{\squiggle{\E}}

\renewcommand{\at}{\a_t}
\newcommand{\atp}{\a_{t+1}}

\newcommand{\pred}{{\hat{a}}}
\newcommand{\predt}{{\pred_t}}

\newcommand{\Q}{\Phi}
%\newcommand{\q}{\phi}

\renewcommand{\z}{\vect{z}}
\newcommand{\zs}{\tilde{\z}}
\renewcommand{\r}{\vect{r}}

\newcommand{\lt}{{L_t}}
\newcommand{\lot}{{L_{1..t}}}
\newcommand{\loT}{{L_{1..T}}}
\newcommand{\lotm}{{L_{1..t-1}}}
\renewcommand{\lq}{{L_q}}

\renewcommand{\thefootnote}{\fnsymbol{footnote}}

